Ordinal Regression as Structured Classification

This paper extends the class of ordinal regression models with a structured interpretation of the problem by applying a novel treatment of encoded labels. The net effect of this is to transform the underlying problem from an ordinal regression task to a (structured) classification task which we solve with conditional random fields, thereby achieving a coherent and probabilistic model in which all model parameters are jointly learnt. Importantly, we show that although we have cast ordinal regression to classification, our method still fall within the class of decomposition methods in the ordinal regression ontology. This is an important link since our experience is that many applications of machine learning to healthcare ignores completely the important nature of the label ordering, and hence these approaches should considered naive in this ontology. We also show that our model is flexible both in how it adapts to data manifolds and in terms of the operations that are available for practitioner to execute. Our empirical evaluation demonstrates that the proposed approach overwhelmingly produces superior and often statistically significant results over baseline approaches on forty popular ordinal regression models, and demonstrate that the proposed model significantly out-performs baselines on synthetic and real datasets. Our implementation, together with scripts to reproduce the results of this work, will be available on a public GitHub repository.

==> authors.tex <==


% \author{Anonymous Authors}
% \affiliation{
%     \institution{Institution}
%     \city{City}
%     \country{Country}
% }
% \email{name@institution}

\author{Callum Mann}
\affiliation{
    \institution{University of Bristol}
    \city{Bristol}
    \country{United Kingdom}
}
\email{cm13558@bristol.ac.uk}

\author{Rafael Poyiadzi}
\affiliation{
    \institution{University of Bristol}
    \city{Bristol}
    \country{United Kingdom}
}
\email{rp13102@bristol.ac.uk}

\author{Raul Santos-Rodriguez}
\affiliation{
    \institution{University of Bristol}
    \city{Bristol}
    \country{United Kingdom}
}
\email{enrsr@bristol.ac.uk}

\author{Niall Twomey}
\orcid{0000-0002-3225-2654}
\affiliation{
    \institution{University of Bristol}
    \city{Bristol}
    \country{United Kingdom}
}
\email{niall.twomey@bristol.ac.uk}


==> results/casas.tex <==
\begin{table}[h]
\tiny
\caption{Table of results for the \casas{} dataset.}
\begin{tabular}{llccc}
\toprule
dataset & model &         0/1 Loss &              MAE &              MSE \\
\midrule
\casas{} & \bn{} &  $0.426\pm0.076$ &  $0.698\pm0.138$ &    $1.483\pm0.4$ \\
         & \lr{} &  $0.436\pm0.066$ &  $0.788\pm0.157$ &  $1.835\pm0.506$ \\
         & \ol{} &  $0.499\pm0.064$ &   $0.759\pm0.11$ &  $1.469\pm0.368$ \\
         & \storm{} &   $0.42\pm0.077$ &  $0.674\pm0.151$ &  $1.396\pm0.432$ \\
\bottomrule
\end{tabular}
\label{table:casas}
\end{table}



==> results/dementiabank.tex <==
\begin{table}[h]
\tiny
\caption{Table of results for the \dementiabank{} dataset.}
\begin{tabular}{llccc}
\toprule
dataset & model &         0/1 Loss &              MAE &              MSE \\
\midrule
\dementiabank{} & \bn{} &  $0.234\pm0.045$ &   $0.382\pm0.07$ &  $0.678\pm0.128$ \\
                & \lr{} &  $0.228\pm0.042$ &  $0.389\pm0.075$ &   $0.71\pm0.145$ \\
                & \ol{} &  $0.356\pm0.038$ &  $0.456\pm0.053$ &  $0.656\pm0.092$ \\
                & \storm{} &  $0.234\pm0.038$ &  $0.366\pm0.063$ &  $0.631\pm0.121$ \\
\bottomrule
\end{tabular}
\label{table:dementiabank}
\end{table}



==> sections/00_abstract.tex <==
\begin{abstract}
Tasks that exhibit explicit ordering amongst their targets will generally be best modelled with ordinal regression. Although these techniques are widely used in economics, health and social sciences, they are often grounded on (or inhibited by) strict assumptions regarding the topology of the label space. In this paper, we approach ordinal regression by reframing it into a structured problem that can be modelled with conditional random fields in a probabilistic model we call \ac{STORM}. This way of interpreting ordinal regression produces a probabilistic model with greater capacity to learn flexible decision boundaries since the assumptions about the topology of the data are less restrictive, it can be flexibly queried, and produces decision boundaries between categories that conform to the ordinal nature of the problem (\ie decisions, when projected into the instance space, are monotonic). We test the efficacy of our technique against several popular ordinal regression models, and demonstrate that the proposed model significantly out-performs baselines on synthetic and real datasets. Our implementation, together with scripts to reproduce the results of this work, will be available on a public GitHub repository on publication. 

% This paper extends the class of \ac{OR} models with a structured interpretation of the problem by applying a novel treatment of encoded labels. The net effect of this is to transform the underlying problem from an \ac{OR} task to a (structured) classification task which we solve with \acp{CRF}, thereby achieving a coherent and probabilistic model in which all model parameters are learnt and optimised together in a single model. Importantly, we show that although we have cast \ac{OR} to classification, our method still fall within the class of decomposition methods in the \ac{OR} ontology. This is an important link since our experience is that many applications of machine learning to healthcare ignores completely the important nature of the label ordering, and hence these approaches should considered na\"{i}ve in this ontology. We also show that our model is flexible both in how it adapts to data manifolds and in terms of the operations that are available for practitioner to execute. Our empirical evaluation demonstrates that the proposed approach overwhelmingly produces superior and often statistically significant results over baseline approaches. 

\end{abstract}


==> sections/01_old_intro.tex <==
\section{Introduction}
\label{section:introduction}

% \todo[inline]{much too long}

Modern healthcare increasingly relies on automated appraisal of patients, and at least two factors contribute to this: intense growth in the ageing population and its associated financial burden, and incommensurate growth of healthcare industry. Consequently, significant research effort is targeting technological advances and predictive modelling for pervasive and in-home healthcare assessment. Chronic and long-term conditions such as \ac{AD} or \ac{PD} are amongst the diseases that are receiving particular attention by the research community. 

Let us consider \ac{AD} as motivating example. When assessing the current state of \ac{AD}, healthcare professionals utilise one of several well-known assessment questionnaires available, \eg \cite{katz1983assessing,pincus1983assessment,wade1988barthel}. 
These questionnaires are designed to uncover the functional ability of a patient and determine if they are capable of living alone safely. 
For instance, in \cite{pincus1983assessment} 20 questions are listed that probe the degree to which patients can live independently and execute \ac{ADL} and \acp{IADL}. 
A weighting is assigned to each question and to each response, and an objective measure of the cognitive ability of the patient is produced by aggregating all the responses together into a unified score. Non-overlapping intervals on the score are then assigned to categories associated with the diagnosis, \eg a patient that scores between, say, 1 and 10 is diagnosed as `cognitively healthy' whereas scores larger than 50 may be indicative of `severe' \ac{AD}. 

The standard machine learning approach is based on learning a mapping between samples and categories so that the probability of error is minimised. However, in this case, the categorisation of the scores into their groups is an ordinal operation (e.g., `severe' diagnoses are more extreme than `moderate' and `mild'). Although the vast majority of the experimental literature on ordinal medical domains recast the task into traditional binary or multiclass problems, we argue that ignoring the natural ordering of the categories would lead to suboptimal results. More formally, given a set of labels for the categories $\{A, B, C, D,\dots\}$, we denote their ordering as $\{A \succ B \succ C \succ D \dots\}$ (where $\succ$ indicates the pairwise ranking within the set). 
%From this we can see that the space of labels has explicit structure, and that models operating on this domain should produce predictions that are consistent with this structure. 
Models that are consistent with this structure are referred to as `ordinal models'. %In the limit case of a model where the estimated probability of error is zero, the it does not make a difference to either use a standard or an ordinal classifier. Otherwise, a principled classifier should be producing predictions that are consistent with the underlying ordering of the categories.


In \ac{AD}, there is a recent interest in the study of data collected from \acp{SH} together with cognitive diagnosis. 
\acp{SH} provide a unique and powerful view into daily life and capture several aspects relating to the behaviour of the resident residing within. 
\ac{SH}-based health assessment opens the opportunity for particularly valuable healthcare research since the unobtrusive manner of data acquisition in smart home yields objective views into the daily behaviour of persons within the smart home. 
In contrast, self-reporting of daily behaviour is well-known to be unreliable. 
The hypothesis of this research area is that the behaviour of a person with \ac{AD} and their interaction with a residential environment will differ in its statistical distribution from that of a non-sufferer of \ac{AD}. 
%This knowledge can be exploited by statistical classifiers and predictive models can be deployed to predict \acp{ADL} and cognitive ability thereafter. 
Recently, researchers have begun to explore these ideas for the purposes of automatically assessing the state of cognitive ability on suffers of \ac{AD}. 
For example, in \cite{dawadi2013automated} the authors recruited 400 participants to perform \acp{IADL} in a smart home that was equipped with environmental sensors. Additionally, in \cite{urwyler2017cognitive} the authors deployed sensor networks in 10 homes of persons with dementia and to 10 further homes of age-matched healthy controls. Interestingly, in these two cases non-ordinal models were selected. 
In the case of \cite{dawadi2013automated} traditional classifiers were used on the ordinal domain, and with \cite{urwyler2017cognitive} the task was recast as a binary classification problem. 
%This is not unusual in the field, and for the majority of the literature on predictive models applied to ordinal tasks areas reviewed by the authors the ordinal nature of the labels was not considered. 
% As well as being prominent in the healthcare field, ordinal tasks can also be found in information retrieval \cite{chu2005gaussian}, bioinformatics \cite{tutz2003generalized}, recommendation systems \cite{koren2011ordrec}, stock analysis \cite{harrell2015regression}, urban planning \cite{alterman1978implementation}, income assessment \cite{mccullagh1980regression}, and grading \cite{chu2005new}. 
% For a review, see \cite{gutierrez2016ordinal}. 

The aims and contributions of this paper, as well as the structure, are as follows: 
We strongly advocate the selection of ordinal techniques for ordinal problems and  a review of ordinal approaches in Section \ref{section:related_work}. 
We introduce a new class of ordinal regression model that is based on a structural interpretation of the field (Section \ref{section:methods}) and demonstrate its utility in our results (Section \ref{section:results}). 
The advantage of the structural interpretation on ordinal regression is that significantly more flexibility is ascribed, and this flexibility permits the model to operate efficiently on linear and non-linear data manifolds. 
Additionally, this interpretation captures contextual information that the other baselines cannot, since, during learning and in prediction, beliefs about all states are propagated within the structure. 
We summarise our work and conclude in Section \ref{section:conclusion}. 


% The main contributions are as follows. 
% We provide a brief review of ordinal classification baselines (Section \ref{section:related_work}), and justify our recommendations for ordinal approaches experimentally (Section \ref{section:results}). 
% This paper also introduces a new class of probabilistic ordinal regression (Section \ref{section:methods}) that we show to be closely related to \acp{CRF}. 
% We outline several synthetic, real, and healthcare datasets (Section \ref{section:experiments}) which we experiment over, and in Section \ref{section:results} we we demonstrate how our model adapts can naturally to non-linear data manifolds and how we out-perform our baselines. 


% \noindent\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}

% Consider a predictive application in which a classifier must make predictions from the following set of labels: $\{\text{very poor}, \text{poor}, \text{no opinion}, \text{good}, \text{excellent}\}$.
% One may simply utilise conventional multiclass machine learning models to learn the mapping from the data to this space of labels, and several model classes, including decision trees, \acp{SVM}, (deep) neural networks, might be viable options in this setting.
% Indeed, flexible and effective predictors can be produced due to the latent representational power of these classifiers. 
% However, these models also assume that the label space of the data is arbitrary, and this assumption is not held with the labels mentioned above. 
% Moreover the ordinal nature of the task imposes a strict structure on the space of labels, namely (and with abuse of notation) that $\text{excellent} > \text{good} > \text{no opinion} > \text{poor} > \text{very poor}$, and if this ordering is not understood by the model one can obtain inconsistent predictors. 

% In the vast majority of published literature on ordinal application areas reviewed by the authors, the ordinal nature of the labels is neglected by practitioners. 
% We argue that the pairing between ordinal data and non-ordinal models is not optimal and we advocate the selection of a more appropriate model classes on these tasks. 
% Ordinal tasks can be found in many healthcare applications including the assessment of Parkinson's disease \cite{patel2009monitoring}, and the assessment of Alzheimer's disease \cite{asgari2017predicting}, and in much of the literature the ordering is not captured in the models. 
% For example, in \cite{dawadi2013automated} the authors recruited 400 persons to perform \acp{IADL} in a smart home that was equipped with environmental sensors.  
% The cohort that was recruited were all diagnosed as being `cognitively healthy', `mild cognitive impairment', and `sufferer of dementia' by domain experts.
% The authors' task was to predict the cognitive ability of the participants from sensor data, and though the label space lies on a discrete, ordinal spectrum only traditional (non-ordinal) models were considered in their work. 

% In \cite{urwyler2017cognitive} the authors deployed sensor networks in 10 homes of persons with dementia and to 10 further homes of age-matched healthy controls. 
% Over a 20 day period data was collected from a variety of sensors and machine learning algorithms predicted each household as belonging to the `healthy' or `dementia' category. 
% However, since the cognitive ability of the recruited participants was quantified with several dementia assessment questionnaires \cite{katz1983assessing,pincus1983assessment,wade1988barthel} the authors could instead have operated on `healthy', `early dementia', `moderate dementia', `advanced dementia' labels which would have provided a more detailed view into the utility of machine learning algorithms in this domain. 

% It is important to state that our discussion of the aforementioned research derives from our view on the importance and under-utilisation of ordinal regression. 
% We consider the applications to be very important, the methodology and the results of these papers to be reputable and we are not dismissive of the work. 
% In our view, the ideal treatment of these applications is that the ordinal nature of the data would be captured by the model, and this work our aspiration is to motivate this treatment in future. 

% As well as being prominent in the healthcare field, ordinal tasks can also be found in information retrieval \cite{chu2005gaussian}, bioinformatics \cite{tutz2003generalized}, recommendation systems \cite{koren2011ordrec}, stock analysis \cite{harrell2015regression}, urban planning \cite{alterman1978implementation}, income assessment \cite{mccullagh1980regression}, and grading \cite{chu2005new}. 
% For a review, see \cite{gutierrez2016ordinal}. 

% In this paper we consider linear predictors of ordinal regression (\ie models which are linear in their parameters) and show how a unified model can be constructed from a novel interpretation of the labels. 
% This interpretation facilitates a flexible ordinal classifier, but the main techniques in this work are general and can be introduced to (deep) neural networks, Bayesian classifiers, including the \ac{BPM} \cite{herbrich2001bayes}, \ac{GPC} \cite{rasmussen2006gaussian}. 

% The remainder of this paper is ordered as follows: in Section \ref{section:related_work} we outline several ordinal models, Section \ref{section:methods} we derive a structural interpretation of ordinal regression that will be used in the remainder of this paper, in Section \ref{section:experiments} the experimental evaluation framework is discussed, and finally in Section \ref{section:results} we tabulate our results and demonstrate the utility of our framework over competing methods with real and synthetic results. 


==> sections/02_related_work.tex <==
\section{Related Work}
\label{section:related_work}


\subsection{Ordinal Models}

One can view ordinal regression as an intermediate problem lying between regression and classification \cite{winship1984regression}, but ordinal regression has received significantly less attention than both regression and classification. 
Here we will describe the two well-known baseline methods that are used in this paper. We have concerned ourselves only with ordinal methods that are linear in their parameters in this work. Therefore we have not considered other methods in this field, including models based on neural network, \cite{cheng2008neural}, decision tree \cite{kramer2001prediction}, neighbourhood \cite{liu2012neighborhood}, \ac{SVM} \cite{herbrich1999support} and Gaussian process \cite{chu2005gaussian} (for a review of methods see \cite{gutierrez2016ordinal}). 

\subsubsection{Ordered Logit}
The classical ordered logit model \cite{mccullagh1980regression} is a simple model that is commonly used in many fields. 
% These two models are very similar and differ only on the noise distribution. 
% We will consider the ordered logit model only here. 
This model assumes that a real-valued latent variable ($y^*$) is defined by

\begin{align}
    y^* = \w^\top \x + \epsilon
\end{align}

\noindent where $\x \in \mathbb{R}^D$ is a data point, $D$ is the dimensionality of the data, $\w \in \mathbb{R}^D$ is a weight vector, and $\epsilon$ is a noise term following the logistic distribution with zero mean and unit variance. 
Assuming $K$ categories, and a set of $K + 1$ thresholds $\theta_k \in \{\theta_0, \theta_1, \dots, \theta_{K}\}$ (ordered by $\theta_k < \theta_{k+1}$) one can assign a response $y$ according to the interval into which $y^*$ falls with the function $f_k: \mathbb{R} \xrightarrow{}  \{0,1\}$:

\begin{align}
    % y={\begin{cases}
    %     1~~~~{\text{if}}~~\theta_ {0}<y^{*}\leq \theta _{1},\\
    %     2~~~~{\text{if}}~~\theta _{1}<y^{*}\leq \theta _{2},\\
    %     \vdots\\
    %     K~~~~{\text{if}}~~\theta _{{K-1}}<y^{*} \leq \theta_{K}.\end{cases}}
    f_k(y^*) = {\begin{cases}
        1~~~~{\text{if}}~~\theta_ {k-1}<y^{*}\leq \theta _{k}\\
        0~~~~{\text{otherwise}}\end{cases}}
    % ~~~~\text{iff}~~\theta _{k-1}<y^{*}\leq \theta _{k}
\end{align}

Three of the thresholds are fixed ($\theta_0=-\infty$, $\theta_1=0$ and $\theta_K=\infty$) to ensure that the process is identifiable \cite{kevin2012machine}. The probability over the categories is computed by integrating the probability mass that falls between the intervals

\begin{align}
    \label{eq:ordlogprob}
    P(y=k|\mathbf {x} ) &=P(\theta _{k-1}<y^{*}\leq \theta _{k}|\mathbf {x} )\nonumber\\
        &=P(\theta _{k-1}<\mathbf {w}^\top \mathbf {x} +\varepsilon \leq \theta _{k})\nonumber\\
        &=\sigma (\theta _{k}-\mathbf {w}^\top \mathbf {x} )-\sigma (\theta _{k-1}-\mathbf {w} ^\top \mathbf {x} )
\end{align}

\noindent where $\sigma(\cdot)$ is the logistic function (\ie cumulative distribution of the logistic distribution). 
% Using this result, one can easily define the log likelihood of the data and optimise all parameters of the model. 
The log-likelihood and its gradient with respect to the parameters ($\{\w, \theta_2, \theta_3, \dots, \theta_{K-1}\}$) are easily computed and can be optimised with standard optimisation techniques \cite{mccullagh1980regression}. 

One of the main advantages of this model over simpler baselines (such as linear regression) is that the ordinal intervals are optimised during the learning routine and that the intervals can have arbitrary widths.
It is important to understand that the primary assumption underpinning these models is that the data lies on a linear manifold, and in practise this is difficult to guarantee. 
% While a practitioner can extend the data representation (\eg with kernel expansions \cite{shashua2003ranking,herbrich2000large,chu2005gaussian}) in this paper we focus on enabling the models to operate on non-linear manifolds directly. 

% \todo[inline]{shared projection over parameters; same progression between classes. }

\subsubsection{Nested Binary Classifiers}
% Ordinal trends along non-linear data manifolds can be captured by cascades of linear classifiers \cite{frank2001simple}.
A more flexible ordinal model can be produced with cascades of linear classifiers \cite{frank2001simple}.
To achieve this the authors recast the ordinal task into $K - 1$ independent binary classification problems. 
The $k$-th binary problem re-partitions the dataset into two groups; the first group consists of all instances whose label is less than or equal to the value $k$, and the second group consists of all instances with label greater than the value $k$. 
% For example, if $K=5$ the $1$-st classifier partitions learns to classify between $\{1\}$ and $\{2, 3, 4, 5\}$, and the $2$-nd classifier partitions classifies between $\{1, 2\}$ and $\{3, 4, 5\}$, or more formally the $k$-th problem is partitioned as $\{i: 1 \leq i \leq k\}$ \vs $\{i: k < i \leq K - 1\}$. 
% The solution to each problem yields a predictor of $P(Y>k)$ since this is how the sub-problems have been partitioned. 

Using an equivalent rationale to that on Equation \eqref{eq:ordlogprob}, the probability distributions over each partition are unified into a probability distribution over the $K$ categories with the following equation

\begin{align}
    P(Y=k|\x) = P(Y > k-0.5|\x) - P(Y>k+0.5|\x)
\end{align}

\noindent with the base cases $P(y>0.5|\x)\triangleq1$ and $P(y>K|\x)\triangleq0$. 
It is important to remember that while the topology of the predictive distribution over the labels can be non-linear, each of the individual pairwise binary classifiers produces linear decision boundaries. 
% We will see later that this model class does not cope with certain data manifolds that other linear models can. 
Additionally, the $K-1$ models are learnt independently, and only the two classifiers that `neighbour' the correct label are used in prediction. 
Although this method is more flexible than the ordered logit, its parameters are learnt in a greedy fashion and will not be optimal. 

\todo[inline]{- I believe that for the nested binary classifiers (equation 4) the decision boundaries could cross, leading to negative probabilities. How do you deal with this?
}

% A consequence of the recursive partitioning is that class imbalance will be induced in many of the sub-problems. 
% One way of overcoming this would be to dynamically adjust the mis-classification costs \cite{elkan2001foundations} for each partition. 
% However, the authors do not discuss this, and in this work we will not consider mis-classification costs.


\subsection{Automated Estimation of Alzheimer’s Disease}

The grounding hypothesis of automating assessment of \ac{AD} is that the data arising from a person with \ac{AD} will differ in its statistical distribution from that of a non-sufferer of \ac{AD}. In a home setting, this may manifest as a difference of interactions with a residential environment  \cite{urwyler2017cognitive}, and in every-day behaviour it may be indicated by a change in spontaneous spoken utterances \cite{asgari2017predicting}. 
% Recently, researchers have begun to explore these ideas for the purposes of automatically assessing the state of cognitive ability on suffers of \ac{AD} in \acp{SH}. 
For example, in \cite{dawadi2013automated} the authors recruited 400 participants to perform \acp{IADL} in a smart home that was equipped with environmental sensors. 
% \ac{AD} models were build on domain knowledge of the home environment, but using regular multi-class classification algorithms the authors were able to predict behaviour. 
In related work \cite{urwyler2017cognitive} researchers deployed sensor networks in 10 homes of persons with dementia and to 10 further homes of age-matched healthy controls. Interestingly, in both of these cases non-ordinal models were used by the authors. 
In the case of \cite{dawadi2013automated} traditional classifiers were used on the ordinal domain, and with \cite{urwyler2017cognitive} the task was recast as a binary classification problem. 
% This is not unusual in the field, and for the majority of the literature on predictive models applied to ordinal tasks areas reviewed by the authors the ordinal nature of the labels was not considered. 
As well as estimating the effects of \ac{AD} on in-home activity and behaviour, researchers have also considered its effect on everyday speech and the potential to separate a cognitively intact healthy control from \ac{MCI} patients in the wild \cite{asgari2017predicting}. \ac{LIWC} features were extracted from textual transcripts and the authors demonstrated predictive accuracy approximately 50\% higher than chance. 
% As well as being prominent in the healthcare field, ordinal tasks can also be found in information retrieval \cite{chu2005gaussian}, bioinformatics \cite{tutz2003generalized}, recommendation systems \cite{koren2011ordrec}, stock analysis \cite{harrell2015regression}, urban planning \cite{alterman1978implementation}, income assessment \cite{mccullagh1980regression}, and grading \cite{chu2005new}. 

